A storm is Coming: A Modern Probabilistic Model Checker

We launch the new probabilistic model checker storm. It features the analysis of discrete- and continuous-time variants of both Markov chains and MDPs. It supports the PRISM and JANI modeling languages, probabilistic programs, dynamic fault trees and generalized stochastic Petri nets. It has a modular set-up in which solvers and symbolic engines can easily be exchanged. It offers a Python API for rapid prototyping by encapsulating storm's fast and scalable algorithms. Experiments on a variety of benchmarks show its competitive performance.

==> fig/modeltypes.tex <==
\begin{wrapfigure}{r}{3cm}
  \begin{tikzpicture}[]
    \tikzstyle{model}=[]
    \node[model] (dtmc) {DTMCs};
    \node[model, right=0.4cm of dtmc] (ctmc) {CTMCs};
    \node[model, above=0.7cm of dtmc] (mdp) {MDPs};
    \node[model, above=1.5cm of ctmc] (ma) {MA};
    
    \node[below=-0.15cm of dtmc, align=center, text width=1.7cm] {\scriptsize \textsl{discrete} \\[-0.15cm] \textsl{probabilities}};

    \node[below=-0.15cm of ctmc, align=center, text width=1.7cm] {\scriptsize \textsl{exponential} \\[-0.15cm] \textsl{delays}};
    
    \draw (dtmc) -- node[left, align=right, text width=2cm] {\scriptsize \textsl{+nondeter-} \\[-0.15cm] \textsl{minism}} (mdp);
    \draw (mdp) -- (ma);
    \draw (ctmc) -- (ma);
  \end{tikzpicture}
  \caption{Supported model types.}
  \label{fig:modeltypes}
\end{wrapfigure}
%
%\begin{table}
%  \def\arraystretch{1.3}\tabcolsep=10pt
%  \begin{center}
%    \caption{Model types supported by \storm.}
%    \begin{tabular}{ccc}
%      \toprule
%      & discrete-time & continuous-time \\
%      \cmidrule{1-3}
%      deterministic & DTMCs & CTMCs \\
%      nondeterministic & MDPs & MA \\
%      \bottomrule
%    \end{tabular} 
%    \label{tab:modeltypes}
%  \end{center}
%\end{table}
